Training Humans to Train Robots Dynamic Motor Skills

Learning from demonstration (LfD) is commonly considered to be a natural and intuitive way to allow novice users to teach motor skills to robots. However, it is important to acknowledge that the effectiveness of LfD is heavily dependent on the quality of teaching, something that may not be assured with novices. It remains an open question as to the most effective way of guiding demonstrators to produce informative demonstrations beyond ad hoc advice for specific teaching tasks. To this end, this paper investigates the use of machine teaching to derive an index for determining the quality of demonstrations and evaluates its use in guiding and training novices to become better teachers. Experiments with a simple learner robot suggest that guidance and training of teachers through the proposed approach can lead to up to 66.5% decrease in error in the learnt skill.

==> Marina_project1 (Version 13723)/ext/tex/abbreviations.tex <==
% define global abbreviations (i.e., used across papers) below
\usepackage{xspace}
\providecommand{\newabbreviation}[2]{#1\ (\renewcommand{#1}{#2\xspace}#1)}

% months
\providecommand{\jan      }{January}
\providecommand{\feb      }{February}
\providecommand{\mar      }{March}
\providecommand{\apr      }{April}
\providecommand{\may      }{May}
\providecommand{\jun      }{June}
\providecommand{\jul      }{July}
\providecommand{\aug      }{August}
\providecommand{\sep      }{September}
\providecommand{\oct      }{October}
\providecommand{\nov      }{November}
\providecommand{\dec      }{December}

% King's
\providecommand{\KCL    }{King's College London}
\providecommand{\NMS    }{Natural and Mathematical Sciences}
\providecommand{\CORE   }{the Centre for Robotics Research}
\providecommand{\RLL    }{Robot Learning Lab}
\providecommand{\WLab   }{Wheatstone Innovation Lab}

% Universities/research institutes
\providecommand{\TUM    }{Technische Universit\"{a}t Munich}
\providecommand{\UKZN   }{University of KawaZulu Natal}
\providecommand{\MIT    }{Massachusetts Institute of Technology}

% funding bodies/schemes
\providecommand{\ERC    }{European Research Council}
\providecommand{\EPSRC  }{Engineering and Physical Sciences Research Council}
\providecommand{\CC     }{Crafts Council}
\providecommand{\JSPS   }{Japan Society for the Promotion of Science}
\providecommand{\AHDB   }{Agriculture and Horticultural Development Board}
\providecommand{\RSSB   }{Rail Safety and Standards Board}
\providecommand{\CONACYT}{Consejo Nacional de Ciencia y Tecnologia}
\providecommand{\HZOZO  }{Horizon 2020}
\providecommand{\FPZ    }{Seventh Framework Program}
\providecommand{\KTP    }{Knowledge Transfer Partnership}
\providecommand{\RIA    }{Research and Innovation Action}
\providecommand{\NIHR   }{National Institute of Health Research}
\providecommand{\DoH    }{Department of Health}
\providecommand{\GCRF   }{Global Challenges Research Fund}
\providecommand{\CTF    }{College Teaching Fund}

% other bodies
\providecommand{\IEEE   }{IEEE}

% journals, conferences
\providecommand{\TRo      }{\IEEE\ \TransactionsOn\ Robotics}
\providecommand{\TNSRE    }{\IEEE\ \TransactionsOn\ Neural \Systems\ \And\ \Rehabilitation\ \Engineering}
\providecommand{\TMech    }{\IEEE\ \TransactionsOn\ Mechatronics}
\providecommand{\IJRR     }{\International\ Journal of Robotics Research}
\providecommand{\NC       }{Neural Computation}
\providecommand{\AURO     }{Autonomous Robots}
\providecommand{\RAL      }{\IEEE\ Robotics \And\ Automation Letters}
\providecommand{\ICRA     }{\IEEE\ \International\ \ConferenceOn\ Robotics and Automation}
\providecommand{\IROS     }{\IEEE\ \International\ \ConferenceOn\ Intelligent Robots and Systems}
\providecommand{\EMBC     }{EMBS/\IEEE\ \International\ \ConferenceOf\ the \Engineering\ in Medicine \And\ Biology \Society}
\providecommand{\RSS      }{Robotics: Science and Systems}
\providecommand{\Humanoids}{\IEEE\ \International\ \ConferenceOn\ Humanoid Robots}
\providecommand{\AIM      }{ASME/\IEEE\ \International\ \ConferenceOn\ Advanced Intelligent Mechatronics}
\providecommand{\ICORR    }{\IEEE\ \International\ \ConferenceOn\ \Rehabilitation\ Robotics}
\providecommand{\BioRob   }{\IEEE\ \International\ \ConferenceOn\ Biomedical Robotics \And\ Biomechatronics}
\providecommand{\NIPS     }{Advances in Neural Information Processing Systems}
\providecommand{\ESANN    }{European Symposium on Artificial Neural Networks}

% people
\providecommand{\PI     }{principle investigator}
\providecommand{\CoI    }{co-investigator}
\providecommand{\RCoI   }{researcher co-investigator}
\providecommand{\PDRA   }{postdoctoral research assistant}
\providecommand{\UG     }{undergraduate}
\providecommand{\PG     }{postgraduate}
\providecommand{\TA     }{teaching assistant}
\providecommand{\MH     }{Matthew Howard}

% certificates/qualifications
\providecommand{\BSc}    {BSc}
\providecommand{\MSci}   {MSci}
\providecommand{\MSc}    {MSc}
\providecommand{\PhD}    {PhD}
\providecommand{\PGCAPHE}{Postgraduate Certificate in Academic Practice in Higher Education}

% machine learning
\providecommand{\RL     }{reinforcement learning}
\providecommand{\HMMs   }{hidden Markov models}

% robotics
\providecommand{\RAS    }{Robotics and autonomous systems}
\providecommand{\ROS    }{Robot Operating System}
\providecommand{\PbD    }{programming by demonstration\xspace}
\providecommand{\DoF    }{degrees of freedom\xspace}
\providecommand{\VIA    }{variable impedance actuator}
\providecommand{\EMG    }{electromyography}
\providecommand{\ECG    }{electrocardiography}
\providecommand{\EEG    }{electroencephalography}
\providecommand{\VPSA   }{variable physical stiffness actuator}
\providecommand{\CCL    }{constraint consistent learning}

% bibliographies
\providecommand{\Journal       }{Journal}
\providecommand{\JournalOf     }{Journal of}
\providecommand{\ConferenceOf  }{Conference of}
\providecommand{\ConferenceOn  }{Conference on}
\providecommand{\TransactionsOn}{Transactions on}
\providecommand{\International }{International}
\providecommand{\And           }{and}
\providecommand{\Rehabilitation}{Rehabilitation}
\providecommand{\Society       }{Society}
\providecommand{\Systems       }{Systems}
\providecommand{\Engineering   }{Engineering}

% general
\providecommand{\WP     }{work package}
\providecommand{\TRL    }{technology readiness level}
\providecommand{\SME    }{small and medium enterprise}
\providecommand{\NGO    }{non-governmental organisation}
\providecommand{\OA     }{open access}
\providecommand{\ICT    }{information and communication technology}
\providecommand{\HCI    }{human computer interfaces}



==> Marina_project1 (Version 13723)/ext/tex/comments.tex <==
% define simple todo command
%\usepackage{lineno}
\usepackage[normalem]{ulem}                                        % for striking text out
\usepackage{marginnote}
\setlength{\marginparwidth}{1.75cm}
\setlength{\marginparsep}{.1mm}
\usepackage[textwidth=\marginparwidth,colorinlistoftodos]{todonotes}
\providecommand{\tinytodo}[2][]
{\todo[caption={#2}, size=\small, #1]{\renewcommand{\baselinestretch}{0.6}\selectfont#2\par}}

% define colours for to-dos
\colorlet{jb}{red}
\colorlet{mh}{red}
\providecommand{\commentcolourcode}{Comments colour code: 
{\color{mh}MH}} 
\providecommand  {\colorsout}[1]{\bgroup\markoverwith{\textcolor{#1}{\rule[0.5ex]{2pt}{0.4pt}}}\ULon} % define coloured strike out
\providecommand{\atMH} {{\color{mh}@MH}}
\providecommand{\atJB} {{\color{jb}@JB}}

\providecommand  {\done}   [1]{\sout{#1}}
\providecommand  {\edit}   [3]{\colorsout{#3}{#1}{\color{#3}{#2}}}
\providecommand  {\nomment}[2]{\tinytodo[color=white,nolist,linecolor=#2,bordercolor=white,noinline]{\protect{\scriptsize\color{#2}#1}}}
\providecommand  {\note}[2]{\tinytodo[color=white,linecolor=#2,bordercolor=white,noinline]{\protect{\scriptsize\color{#2}#1}}}
%\providecommand  {\at}     [1]{\textcolor{#2}{@#2}}


\providecommand{\makecomments}{%
\section*{Usage notes}~\\%[1ex]
\noindent Use \texttt{\textbackslash note\{your comment\}\{your initials\}} to add comments/to dos. For example,
\underline{J}oe \underline{B}loggs adds comments using \texttt{\textbackslash note\{Comment.\}\{jb\}}.\nomment{These comments will appear as margin notes. They will also appear in the todo list on the first page.}{jb} \\[2ex]
%\noindent Optionally, use \texttt{\textbackslash atInitials} to address your comment to someone (\eg \texttt{\textbackslash note\{\textbackslash atJB: Please fix this.\}\{mh\}}).\\[2ex]
You can mark a comment as resolved using \texttt{\textbackslash done\{Comment text.\}}, (\eg \texttt{\textbackslash note\{\textbackslash done\{\textbackslash atJB: Please fix this.\}\}\{mh\}}). It will then be formatted like this: \done{\atJB: Please fix this.}.\\[2ex]
\commentcolourcode\\[1ex]
\printacronyms~\\[2ex]% if using glossaries package to manage acronyms, print them
\listoftodos~\\[2ex]
\clearpage\setcounter{page}{1}
%\linenumbers%
}

\providecommand{\makenotes}{\clearpage\appendix\input{notes}}%

\providecommand{\makefinal}{%
\renewcommand{\makecomments}{}\renewcommand{\makenotes}{}\renewcommand{\note}[1]{}\renewcommand{\done}[1]{}\renewcommand{\edit}[3]{\#2}\renewcommand{\comment}[2]{}%
}


==> Marina_project1 (Version 13723)/ext/tex/format.tex <==
\usepackage{xspace}

% define format of some common idioms
\providecommand{\eg}{\textit{e.g.,}~} %
\providecommand{\ie}{\textit{i.e.,}~} %
\providecommand{\qv}{\textit{q.v.,}~} %
\providecommand{\apriori}{\textit{a~priori}\xspace} %
\providecommand{\etc}{\textit{etc.}} %
\providecommand{\naive}{na\"ive\xspace} %

% define format of numbers
\providecommand{\thousand}{k} %
\providecommand{\million} {m} %
\providecommand{\billion}{bn} %

% define page/section/figure/table/etc. referencing format
\providecommand*{\pref}[1]{p.\pageref{#1}}          % page
\providecommand*{\sref}[1]{\S\ref{s:#1}}            % section
\providecommand{\tablename}{Table}
\providecommand*{\tref}[1]{\tablename~\ref{t:#1}}   % table
\providecommand{\figurename}{Fig.}
\providecommand*{\fref}[1]{\figurename~\ref{f:#1}}  % figure
\providecommand*{\eref}[1]{(\ref{e:#1})}            % equation

% define list formatting
\let\labelindent\relax %<-this prevents a conflict with IEEE \labelindent when using enumitem
\usepackage[inline]{enumitem} % use enumitem package to get inline lists, set the list format
\setlist{nolistsep}
\providecommand{\il}[1]{\begin{enumerate*}[label=(\roman*)]#1\end{enumerate*}} % inline list (for use in main text)
\providecommand{\cl}[1]{\begin{enumerate*}[label=(\alph*)]#1\end{enumerate*}}  % caption list (for use in captions)



==> Marina_project1 (Version 13723)/ext/tex/symbols.tex <==
% define global symbols (i.e., for use across papers) below
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{gensymb}

% character definition
\mathchardef\mhyphen="2D   % define "math hyphen"

% equivalence relations
\providecommand{\defeq}{\vcentcolon=}

% maths
\providecommand{\R}     {\mathbb{R}}          % real numbers
\providecommand{\T}     {\top}                % transpose
\providecommand{\intd}  {\mathrm{d}}          % variable of integration
\providecommand{\bO}    {\boldsymbol{0}}      % (bold) zero
\providecommand{\bl}    {\boldsymbol{1}}      % (bold) one
\providecommand{\bnabla}{\boldsymbol{\nabla}} % (bold) derivative
\providecommand{\N}     {\mathcal{N}}         % Gaussian distribution
\providecommand{\U}     {\mathcal{U}}         % uniform distribution
\providecommand{\I}     {\mathbf{I}}          % identity matrix
\providecommand{\be}    {\mathbf{e}}          % basis vector

% functions
\providecommand{\estimated} [1]{\tilde{#1}}
\providecommand{\normalised}[1]{\hat{#1}}
\providecommand{\optimal}   [1]{\bar{#1}}
\providecommand{\pinv}      [1]{{#1}^\dagger}
\providecommand{\vectornorm}[1]{||#1||}
\providecommand{\trace}     [1]{\mathrm{Tr}[#1]}        % pseudoiverse quantity
\providecommand{\leftexp}   [2]{{\vphantom{#2}}^{#1}{#2}}

% indices
\providecommand{\nd}      {n}                              % index for data points
\providecommand{\nk}      {k}                              % index for task spaces
\providecommand{\Nd}      {\mathcal{\MakeUppercase{\nd}}}  % no. data points
\providecommand{\Nk}      {\mathcal{\MakeUppercase{\nk}}}  % no. task spaces

% inputs/outputs
\providecommand{\x}      {x}                  % state
\providecommand{\bx}     {\mathbf{x}}         % (bold) state
\providecommand{\nx}     {p}                  % index for elements of input/state vector
\providecommand{\dimx}   {\mathcal{\MakeUppercase{\nx}}} % input/state dimensionality
\providecommand{\by}     {\mathbf{y}}         % (bold) output/observation
\providecommand{\ny}     {r}                  % index for elements of output/observation vector
\providecommand{\dimy}   {\mathcal{\MakeUppercase{\ny}}} % output/observation dimensionality

% parameters
\providecommand{\btheta}  {\boldsymbol{\theta}}               % parameter vector
\providecommand{\ntheta}  {p}                                 % index for parameter vector elements
\providecommand{\dimtheta}{\mathcal{\MakeUppercase{\ntheta}}} % parameter dimensionality

% constrained systems
\providecommand{\bA}     {\mathbf{A}}         % constraint matrix
\providecommand{\bb}     {\mathbf{b}}         % constraint vector
\providecommand{\nb}     {s}                  % index for elements of b
\providecommand{\dimb}   {\mathcal{\MakeUppercase{\nb}}} % observation dimensionality
\providecommand{\bN}     {\mathbf{N}}         % null space projection matrix
\providecommand{\bc}     {\mathbf{c}}         % null space vector
\providecommand{\dimc}   {\dimy}              % dimensionality of null space vector
\providecommand{\bw}     {\mathbf{w}}         % image space part
\providecommand{\dimw}   {\dimy}              %
\providecommand{\bv}     {\mathbf{v}}         % null space part
\providecommand{\dimv}   {\dimy}              %

% kinematics
\providecommand{\q}      {q}                  % joint angles
\providecommand{\bq}     {\mathbf{\q}}        % (bold) joint angles
\providecommand{\br}     {\mathbf{r}}         % (bold) end-effector positions
\providecommand{\nr}     {q}                  % index for elements of end-effector position vector
\providecommand{\dimr}   {\mathcal{\MakeUppercase{\nr}}} %  end-effector position vector dimensionality
\providecommand{\bJ}     {\mathbf{J}}         % Jacobian
\providecommand{\qdot}   {\dot{q}}            % joint velocities
\providecommand{\bqdot}  {\dot{\bq}}          % (bold) joint velocities
\providecommand{\rdot}   {\dot{r}}            % end-effector velocities
\providecommand{\brdot}  {\dot{\br}}          % (bold) end-effector velocities
\providecommand{\ebq}    {\estimated{\bq}}    % (bold) estimated joint angles
\providecommand{\ebqdot} {\estimated{\bqdot}} % (bold) estimated joint velocities

% dynamics
\providecommand{\bF}     {\mathbf{f}}         % (bold) force
\providecommand{\qddot}  {\ddot{q}}           % joint accelerations
\providecommand{\bqddot} {\ddot{\bq}}         % (bold) joint accelerations
\providecommand{\btau}   {\boldsymbol{\tau}}  % (bold) joint torques
\providecommand{\ebqddot}{\estimated{\bqddot}}% (bold) estimated joint accelerations
\providecommand{\ebtau}  {\estimated{\btau}}  % (bold) estimated joint torques
\providecommand{\rddot}  {\ddot{r}}           % end-effector accelerations
\providecommand{\brddot} {\ddot{\br}}         % (bold) end-effector accelerations
\providecommand{\bK}     {\mathbf{K}}         % (bold) stiffness matrix
\providecommand{\bB}     {\mathbf{B}}         % (bold) damping matrix
\providecommand{\brO}    {\br_{0}}            % (bold) equilibrium position in Cartesian space

% control
\providecommand{\u}      {u}                  % input/command

\providecommand{\bu}     {\mathbf{\u}}        % (bold) input/command
\providecommand{\nu}     {q}                  % index for elements of u
\providecommand{\dimu}   {\mathcal{\MakeUppercase{\nu}}} % action dimensionality
\providecommand{\bpi}    {\boldsymbol{\pi}}   % (bold) control policy
\providecommand{\bxdot}  {\dot{\bx}}          % (bold) state velocities

% learnt models
\providecommand{\bm}     {\mathbf{m}}         % (bold) RBF or local model centres
\providecommand{\bxn}    {\bx_{\nd}}          % nth input data point
\providecommand{\byn}    {\by_{\nd}}          % nth output data point
\providecommand{\bX}     {\mathbf{X}}         % input data matrix
\providecommand{\bU}     {\mathbf{U}}         % output data matrix

% regression/classification
\providecommand{\bphi}  {\boldsymbol{\phi}}               % feature vector
\providecommand{\bPhi}  {\boldsymbol{\Phi}}               % 
\providecommand{\nphi}  {s}                               % index for feature vector elements
\providecommand{\dimphi}{\mathcal{\MakeUppercase{\nphi}}} % feature dimensionality
\providecommand{\numD} {\mathcal{N}} % number of data points

\providecommand{\wAngle} {\mathcal{\omega}}  % angle between data points
\providecommand{\magnitude} {c}  % magnitude of data points
\providecommand{\bwAngle}  {\boldsymbol{\omega}}


% reinforcement learning

% generic symbols

% equations

% learning algorithm
\providecommand{\A}     {\mathcal{A}} 
\providecommand{\D}     {\mathbf{D}} 
%\providecommand{\model}     {\mathbf{\theta}} 



% other






==> Marina_project1 (Version 13723)/tex/abbreviations.tex <==
% include global abbreviations
\input{ext/tex/abbreviations}

\usepackage[acronym]{glossaries}%
\glsdisablehyper % switch off hyperlinks for abbreviations
\makeglossaries%
\providecommand{\ab}[1]{\gls{#1}}

% define local abbreviations (i.e., for this paper) below
\newacronym{lfd}{LfD}{Learning from demonstration}
\newacronym{mt}{MT}{machine teaching}
\newacronym{nmse}{NMSE}{normalised mean squared error}
\newacronym{ols} {OLS} {ordinary least squares}
\newacronym{lip}{LiP}{linear-in-the-parameters}



==> Marina_project1 (Version 13723)/tex/comments.tex <==
\input{ext/tex/comments}

% define commands for each author
\colorlet{ma}{blue}

\renewcommand{\commentcolourcode}{Comments colour code: 
 {\color{mh}MH}%
,{\color{ma}MA}%
} 

 % shortcut commenting commands
\providecommand{\mh}[1]{\note{#1}{mh}}
\providecommand{\mhcn}{\note{Citation needed.}{mh}} % shortcut commenting commands


==> Marina_project1 (Version 13723)/tex/format.tex <==
% include global formatting definitions
\input{ext/tex/format}

% define local formatting definitions  (i.e., for this paper) below


% deal with bad hyphenation
\hyphenation{public-ations}



==> Marina_project1 (Version 13723)/tex/preamble.tex <==
\usepackage{times}
\usepackage{graphicx}\graphicspath{{img/}}
\usepackage{epstopdf}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{multirow} 
\usepackage{multicol}
\usepackage{array}
\usepackage{mdwmath}
\usepackage{mdwtab}
\usepackage{rotating}
\usepackage[list=off]{caption}
\usepackage{amssymb}
\usepackage{verbatim}
\usepackage{overpic}
\usepackage{amsmath}
\usepackage{subcaption}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[export]{adjustbox}
%\usepackage{hyperref}
\usepackage[normalem]{ulem}
\usepackage{siunitx} % for formatting units
\usepackage{chngpage}
%\usepackage{comment}

\input{tex/abbreviations}
\input{tex/symbols}
\input{tex/format}
\input{tex/comments}

% set up manual labelling
\makeatletter\newcommand{\manuallabel}[2]{\def\@currentlabel{#2}\label{#1}}\makeatother

\usepackage[
backend=bibtex,
style=ieee,
url=false,
doi=false,
isbn=false,
doi=true,
eprint=false
]{biblatex}
\addbibresource{bib/abbreviations.bib}
\addbibresource{bib/bibliography.bib}
\renewcommand*{\bibfont}{\footnotesize}% set fontsize to match that of ieeeconf



==> Marina_project1 (Version 13723)/tex/symbols.tex <==
% include global symbols
\input{ext/tex/symbols}

\providecommand{\activationfunction}     {\boldsymbol{\phi}} 


% define local symbol definitions (i.e., for this paper) below
\providecommand{\model}{\boldsymbol{\theta}}  % model

\providecommand{\target}{{\boldsymbol{\theta}^*}}  % target model

\providecommand{\learnt}{\estimated{\boldsymbol{\theta}}}  % learnt model
\providecommand{\learntaction}{\estimated{\action}}  % learnt model

\providecommand{\dataset}{\boldsymbol{\mathcal{D}}} % dataset

\providecommand{\teaching}     {\mathcal{T}} % teaching strategy

\providecommand{\feedbackf}     {\mathcal{G}} % feedback function


\providecommand{\feedback}     {f} % feedback

\providecommand{\guidance}     {g} % feedback

\providecommand{\query}     {q} % queries

\providecommand{\argmin}{\mathop{\rm arg~min}\limits}



\providecommand{\searchspaceD}{\boldsymbol{\mathfrak{D}}} % search space of dataset

%\providecommand{\searchspaceM}{\boldsymbol{\mathfrak{\theta}}} % search space of model
\providecommand{\searchspaceM}{\boldsymbol{\mathfrak{Q}}} % search space of model

\providecommand{\action}{u}  % torque/action

\providecommand{\state}{\boldsymbol{x}}         % (bold) state 

\providecommand{\actions}{\boldsymbol{u}}  % torque/action matrix

\providecommand{\states}{\boldsymbol{X}}         % (bold) state matrix

\providecommand{\W}{\boldsymbol{W}}         % (bold) W matrix

\providecommand{\orth}{\boldsymbol{P}}         % (bold) P matrix

\providecommand{\B}{\boldsymbol{B}}         % (bold) B matrix


\providecommand{\noisevar}{\mathcal{\noisestd}^2}  % variance
\providecommand{\noisestd}{\mathcal{\sigma}}  % standard deviation
%\providecommand{\noisestd}{\mathcal{\sigma}_n}  % standard deviation

\providecommand{\reg}      {\mathcal{\lambda}}
\providecommand{\eig}      {b}


\providecommand{\featuref}  {\boldsymbol{\mathcal{\phi}}}    % basis function

\providecommand{\triskf}  {\mathcal{\rho}}    % teaching risk function

\providecommand{\terrorf}  {\mathcal{\varepsilon}}    % teaching error function

\providecommand{\rmse}  {\mathnormal{E_{RMSE}}} 
\providecommand{\nmse}  {\mathnormal{E_{NMSE}}}
\providecommand{\ltwonorm}  {\mathnormal{E_{l2}}}



\providecommand{\length}      {l}   %length
\providecommand{\mass}      {m}   %mass
\providecommand{\gravity}      {g}   %gravity





\providecommand{\wstar}{\mathbf{w}^*}             % target parameter
\renewcommand  {\Nd}      {N}                     % (redefined) number of data points

\renewcommand  {\u}       {y}                     % input/command
\renewcommand  {\xi}      {q}           % first state variable
\providecommand{\xii}     {\dot{q}}           % second state variable
\providecommand{\bepsilon}{\boldsymbol{\epsilon}} % noise on state
\providecommand{\stiffness}{k}            % damping
\providecommand{\damping}{d}            % damping coefficient 

\providecommand{\bTheta}  {\boldsymbol{\Theta}}   % parameter matrix
\providecommand{\e}       {e}                     % element of basis (orthonormal unit) vector
\providecommand{\be}      {\mathbf{\e}}           % basis (orthonormal unit) vector

\providecommand{\bPsi}  {\boldsymbol{\Psi}}               % 
\providecommand{\rotation}  {\boldsymbol{R}}               % 

 
\providecommand{\n}{??}
\providecommand{\bY}{??}
\DeclareUnicodeCharacter{0308}{??}

\providecommand{\score}{s}

\FPset{\trialsi}{500} % trials of experiment 1

%\providecommand{\mean}{\mu}    % mean in experimental data analysis
%\providecommand{\sd}  {\sigma} % s.d. in experimental data analysis
